Projection onto quadratic hypersurfaces

We address the problem of projecting a point onto a quadratic hypersurface, more specifically a central quadric. We show how this problem reduces to finding a given root of a scalar-valued nonlinear function. We completely characterize one of the optimal solutions of the projection as either the unique root of this nonlinear function on a given interval, or as a point that belongs to a finite set of computable solutions. We then leverage this projection and the recent advancements in splitting methods to compute the projection onto the intersection of a box and a quadratic hypersurface with alternating projections and Douglas-Rachford splitting methods. We test these methods on a practical problem from the power systems literature, and show that they outperform IPOPT and Gurobi in terms of objective, execution time and feasibility of the solution.

==> tags <==
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_PROGRAM_AUTHOR	Darren Hiebert	/dhiebert@users.sourceforge.net/
!_TAG_PROGRAM_NAME	Exuberant Ctags	//
!_TAG_PROGRAM_URL	http://ctags.sourceforge.net	/official site/
!_TAG_PROGRAM_VERSION	5.9~svn20110310	//
2D example of a nondegenerate projection onto a hyperbola	main.tex	/^	Remark that with the knowledge of the value of $\\muI$, we could launch a single Newton scheme with the appropriate starting point. Unfortunately, computing $\\muI$ amounts to computing the root of $f''$ which is at least as costly as finding the root of $f$.$/;"	b
2D example of a nondegenerate projection onto an ellipse	main.tex	/^	\\end{proof}$/;"	b
Acknowledgement	main.tex	/^For the second part of the paper,~\\cref{sec:Splitting_methods}, further research may include the comparison with the alternating projection method using inexact projections, \\eg, projecting on the tangent space of the previous feasible point. Such methods are discussed in~\\cite{drusvyatskiy_local_2019}. %Also, the splitting methods analysed here could be used to project a point onto the feasible set of the ACOPF problem that comes from the power systems literature. This feasible set can be formulated as the intersection between a polytope and quadratic hypersurfaces.$/;"	s
All eigenvalues are distinct	main.tex	/^Let us first assume that all eigenvalues of $\\A$ are distinct, the case with repeated eigenvalues is treated at the end of the current section.$/;"	b
Alternating projection method	main.tex	/^\\end{align}$/;"	u
Alternating projections versus Gurobi	main.tex	/^\\end{figure}$/;"	u
Comparison	main.tex	/^\\end{figure}$/;"	u
Conclusion	main.tex	/^\\end{figure}$/;"	s
Damped alternating projection method	appendix.tex	/^\\end{figure}$/;"	u
Degenerate case  texorpdfstring  $ mathbf  x	main.tex	/^	\\end{figure}$/;"	u
Douglas-Rachford  Alternating Projections and IPOPT	main.tex	/^and is an intuitive measure of how far an infeasible point is to the feasible set. The prescribed tolerance for the deviation is $10^{-6}$. This deviation does not account for the box. This is not an issue here, because none of the tests considered in the numerical experiments terminates outside of the box.$/;"	u
Douglas-Rachford method	main.tex	/^\\end{figure}$/;"	u
Ellipsoid experiments	main.tex	/^From these two experiments, it appears that both DR-F and APE are the methods that find the best solution in terms of objective. However, if the execution time is taken into account, APG reaches an objective close to the one of DR-F and APE in a significantly lower run time. APG should therefore be considered, \\eg, if the eigenvector decomposition is too expensive to compute. APC works particularly well in the ellipsoidal case, but performs worse in the hyperboloidal case. IPOPT is clearly the slowest method. It achieves good solution objectives in the ellipsoidal case, but gives poorer results in the hyperboloidal case.$/;"	b
Exact projection onto quadric in normal form	appendix.tex	/^\\end{enumerate}$/;"	s
Extensions and applications	main.tex	/^\\end{table}$/;"	u
Failure of the quasi-projection	main.tex	/^\\end{algorithm}$/;"	b
Features of the quasi-projection	main.tex	/^\\end{figure}$/;"	b
Formulation of the projection onto the quadric as a standard form	appendix.tex	/^\\appendix$/;"	s
Hyperboloid case  texorpdfstring  $ mathbf  x	main.tex	/^	\\end{figure}$/;"	u
Hyperboloid experiments	main.tex	/^\\end{figure}$/;"	b
Implementation details	main.tex	/^Moreover, the point that has to be projected in~\\cite{vh22} is obtained as the solution of a surrogate problem defined on a relaxed set, see~\\cite{vh19,vh20,vh22} for more details. And because this relaxation is close to the feasible set, the point that has to be projected is inside the box and near the quadric. This is the reason for the favorable performance of APC which is reported in~\\cref{sub:Alternate_projection_versus_Gurobi}.$/;"	u
Introduction	main.tex	/^\\textbf{Keywords}: quadric, quadratic surfaces, nonconvex projection, Douglas-Rachford splitting, alternating projections.$/;"	s
Modified Douglas-Rachford	main.tex	/^\\end{algorithm}$/;"	P
Multiple-shot experiment	main.tex	/^\\end{figure}$/;"	b
Numerical experiments	main.tex	/^Such a restart mechanism is not a guarantee of convergence: the method can then be trapped into another region, or even come back to the exact same region. But in the few instances ($\\approx$ once every 10000 trials) where the presented algorithms experience convergence issues, the restart results in successful convergence.$/;"	s
One-shot experiment	main.tex	/^by a small number of instances that terminate due to a timeout. However, we also record the number of timeouts---either due to maximum iterations or time limit. %---, because a timeout is an undesirable situation that should be recorded.$/;"	b
Projection onto a box	main.tex	/^The structure is the following: \\S~\\ref{sub:Projection_on_the_box} briefly recalls how to project onto a box, \\S~\\ref{sub:Alternate_projection_method_AP} details the AP  methods, and \\S~\\ref{sub:Douglas-Rachford_method} covers the DR splitting. A comparison table of all methods is presented in \\S~\\ref{sub:comparison}, a power systems application is discussed in \\S~\\ref{sub:Extensions_and_further_researches}, and a restart mechanism is given in \\S~\\ref{sub:Implementation_details}.$/;"	u
Quadric is a sphere	appendix.tex	/^\\label{sec:Exact_projection_on_quadric}$/;"	u
Quasi-projection onto the quadric	main.tex	/^\\end{figure}$/;"	u
Splitting methods for the projection onto the intersection of a box and a quadric	main.tex	/^In general the quasi-projection is not exact, in the sense that the resulting point is \\emph{not} the optimal solution of~\\cref{eq:proj_quadric}. However, we expect the quasi-projection to be close to optimality when the point is close enough to the quadric. Such a behaviour is observed in our simulations in~\\cref{sub:Alternate_projection_versus_Gurobi}. Also, in the specific case when the quadric is a sphere, then both $\\mathrm{P}_1$ and $\\mathrm{P}_2$ solve~\\cref{eq:proj_quadric}. $/;"	s
declarations	main.tex	/^\\include{packages}$/;"	i
packages	main.tex	/^}$/;"	i

